Multi-Agent Bayesian Optimization with Coupled Black-Box and Affine Constraints

This paper studies the problem of distributed multi-agent Bayesian optimization with both coupled black-box constraints and known affine constraints. A primal-dual distributed algorithm is proposed that achieves similar regret/violation bounds as those in the single-agent case for the black-box objective and constraint functions. Additionally, the algorithm guarantees an $\mathcal{O}(N\sqrt{T})$ bound on the cumulative violation for the known affine constraints, where $N$ is the number of agents. Hence, it is ensured that the average of the samples satisfies the affine constraints up to the error $\mathcal{O}({N}/{\sqrt{T}})$. Furthermore, we characterize certain conditions under which our algorithm can bound a stronger metric of cumulative violation and provide best-iterate convergence without affine constraint. The method is then applied to both sampled instances from Gaussian processes and a real-world optimal power allocation problem for wireless communication; the results show that our method simultaneously provides close-to-optimal performance and maintains minor violations on average, corroborating our theoretical analysis.

==> figs/ri_cumu_regret.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Step},
xmin=0, xmax=101,
xtick style={color=black},
xtick={0,25,50,75,100,125},
xticklabels={
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\),
  \(\displaystyle {75}\),
  \(\displaystyle {100}\),
  \(\displaystyle {125}\)
},
y grid style={darkgray176},
ylabel={Cumulative Regret},
ymin=-6.196351286858, ymax=21.755758140862,
ytick style={color=black},
ytick={-10,0,10,20,30},
yticklabels={
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {0}\),
  \(\displaystyle {10}\),
  \(\displaystyle {20}\),
  \(\displaystyle {30}\)
}
]
\path [draw=green, fill=green, opacity=0.3]
(axis cs:0,0.684164572657574)
--(axis cs:0,0.389589783065727)
--(axis cs:1,0.548578293128894)
--(axis cs:2,0.725035145692477)
--(axis cs:3,1.1632618215363)
--(axis cs:4,1.62916531350856)
--(axis cs:5,1.57188280487718)
--(axis cs:6,1.64252210854451)
--(axis cs:7,1.64841535591123)
--(axis cs:8,1.7188101551174)
--(axis cs:9,1.53015612920361)
--(axis cs:10,1.3692108856352)
--(axis cs:11,1.24955337224955)
--(axis cs:12,1.12810024667654)
--(axis cs:13,0.919142943611859)
--(axis cs:14,0.808255800738264)
--(axis cs:15,0.664488629092906)
--(axis cs:16,0.513433404190224)
--(axis cs:17,0.380077284145094)
--(axis cs:18,0.2083014870197)
--(axis cs:19,0.0301033741278376)
--(axis cs:20,-0.159522869873306)
--(axis cs:21,-0.322302639832963)
--(axis cs:22,-0.469373112187843)
--(axis cs:23,-0.61633840137324)
--(axis cs:24,-0.771809605310944)
--(axis cs:25,-0.916005295828113)
--(axis cs:26,-1.08132510812557)
--(axis cs:27,-1.20808211372448)
--(axis cs:28,-1.33855336119556)
--(axis cs:29,-1.48423775834049)
--(axis cs:30,-1.5930774473163)
--(axis cs:31,-1.65378551398774)
--(axis cs:32,-1.79254797562109)
--(axis cs:33,-1.88237308615542)
--(axis cs:34,-2.01613965467871)
--(axis cs:35,-2.10037103736402)
--(axis cs:36,-2.22706957056069)
--(axis cs:37,-2.34357791010244)
--(axis cs:38,-2.47619194305037)
--(axis cs:39,-2.58918692698893)
--(axis cs:40,-2.6902925299727)
--(axis cs:41,-2.80120768677976)
--(axis cs:42,-2.89247853089339)
--(axis cs:43,-3.01464419216797)
--(axis cs:44,-3.08168609252881)
--(axis cs:45,-3.19397789254291)
--(axis cs:46,-3.25636318183628)
--(axis cs:47,-3.32022997039426)
--(axis cs:48,-3.3622397602008)
--(axis cs:49,-3.41212859790153)
--(axis cs:50,-3.45140666826129)
--(axis cs:51,-3.50090041106925)
--(axis cs:52,-3.54827731822284)
--(axis cs:53,-3.59728013840454)
--(axis cs:54,-3.64627953229641)
--(axis cs:55,-3.68939912955543)
--(axis cs:56,-3.71898385601506)
--(axis cs:57,-3.74079072502523)
--(axis cs:58,-3.76679225556307)
--(axis cs:59,-3.81925622359552)
--(axis cs:60,-3.84195554532979)
--(axis cs:61,-3.88048057147933)
--(axis cs:62,-3.90009603302264)
--(axis cs:63,-3.91991912072416)
--(axis cs:64,-3.93397522038101)
--(axis cs:65,-3.97932045842643)
--(axis cs:66,-3.99738412195451)
--(axis cs:67,-4.04276215549663)
--(axis cs:68,-4.07122048201716)
--(axis cs:69,-4.0951565172318)
--(axis cs:70,-4.11815919960538)
--(axis cs:71,-4.16129471940635)
--(axis cs:72,-4.19067695901282)
--(axis cs:73,-4.20768082038266)
--(axis cs:74,-4.23232671464907)
--(axis cs:75,-4.26382829644119)
--(axis cs:76,-4.30023469102109)
--(axis cs:77,-4.32565236347219)
--(axis cs:78,-4.35340716123741)
--(axis cs:79,-4.38943854750972)
--(axis cs:80,-4.41735330983835)
--(axis cs:81,-4.43584402154061)
--(axis cs:82,-4.47083241168179)
--(axis cs:83,-4.49549894662959)
--(axis cs:84,-4.52187794521498)
--(axis cs:85,-4.54080848880736)
--(axis cs:86,-4.57270811909746)
--(axis cs:87,-4.59984999331019)
--(axis cs:88,-4.61618756011833)
--(axis cs:89,-4.63514625718895)
--(axis cs:90,-4.66869602385151)
--(axis cs:91,-4.69149580044113)
--(axis cs:92,-4.71171962762089)
--(axis cs:93,-4.73245757594535)
--(axis cs:94,-4.75946087575547)
--(axis cs:95,-4.79135550179024)
--(axis cs:96,-4.8194025778333)
--(axis cs:97,-4.8362093748948)
--(axis cs:98,-4.86317855140165)
--(axis cs:99,-4.89230271758524)
--(axis cs:100,-4.92580085832527)
--(axis cs:100,1.89081703274973)
--(axis cs:100,1.89081703274973)
--(axis cs:99,1.89245241089102)
--(axis cs:98,1.88881005410076)
--(axis cs:97,1.88291835337196)
--(axis cs:96,1.8643917490679)
--(axis cs:95,1.86038578357712)
--(axis cs:94,1.85604778446487)
--(axis cs:93,1.85305081508053)
--(axis cs:92,1.83988763936323)
--(axis cs:91,1.82806997735672)
--(axis cs:90,1.81641731876276)
--(axis cs:89,1.81939049660563)
--(axis cs:88,1.80443794620856)
--(axis cs:87,1.8071270755598)
--(axis cs:86,1.80202368490546)
--(axis cs:85,1.80312919602018)
--(axis cs:84,1.79234949299723)
--(axis cs:83,1.79033225004111)
--(axis cs:82,1.7848089321429)
--(axis cs:81,1.78904706331669)
--(axis cs:80,1.77676523272624)
--(axis cs:79,1.77611342846181)
--(axis cs:78,1.78307032192174)
--(axis cs:77,1.78203658434993)
--(axis cs:76,1.7745442941496)
--(axis cs:75,1.78385620432986)
--(axis cs:74,1.78736653917248)
--(axis cs:73,1.78356816187356)
--(axis cs:72,1.77236805996967)
--(axis cs:71,1.7758536919878)
--(axis cs:70,1.78898282855023)
--(axis cs:69,1.78808016170101)
--(axis cs:68,1.78404910177528)
--(axis cs:67,1.78721945009544)
--(axis cs:66,1.80651605981714)
--(axis cs:65,1.79787378158537)
--(axis cs:64,1.81212157629465)
--(axis cs:63,1.80048874429188)
--(axis cs:62,1.79341463121916)
--(axis cs:61,1.79287907068039)
--(axis cs:60,1.80573821677515)
--(axis cs:59,1.8055290369822)
--(axis cs:58,1.81914076789199)
--(axis cs:57,1.82200904252424)
--(axis cs:56,1.81945768080571)
--(axis cs:55,1.82980820668277)
--(axis cs:54,1.84628528587631)
--(axis cs:53,1.85493572891004)
--(axis cs:52,1.87076593563614)
--(axis cs:51,1.89651109735843)
--(axis cs:50,1.90296956529082)
--(axis cs:49,1.92515170070918)
--(axis cs:48,1.93222115348253)
--(axis cs:47,1.93500588479862)
--(axis cs:46,1.9527549941184)
--(axis cs:45,1.97353973678973)
--(axis cs:44,1.98829480761412)
--(axis cs:43,2.00640548172709)
--(axis cs:42,2.02864328213959)
--(axis cs:41,2.03935051878821)
--(axis cs:40,2.04944773391895)
--(axis cs:39,2.04492063678225)
--(axis cs:38,2.05528702671836)
--(axis cs:37,2.08339836470954)
--(axis cs:36,2.09738049953451)
--(axis cs:35,2.12097507219278)
--(axis cs:34,2.13761167050212)
--(axis cs:33,2.16979848407312)
--(axis cs:32,2.19183888394684)
--(axis cs:31,2.23111309166446)
--(axis cs:30,2.24136698400394)
--(axis cs:29,2.249882590769)
--(axis cs:28,2.27570382649771)
--(axis cs:27,2.29245968386827)
--(axis cs:26,2.34074422749892)
--(axis cs:25,2.38180898457832)
--(axis cs:24,2.42773663165969)
--(axis cs:23,2.46606989882691)
--(axis cs:22,2.5119007039786)
--(axis cs:21,2.53848438943042)
--(axis cs:20,2.58596949832028)
--(axis cs:19,2.64332171855648)
--(axis cs:18,2.70099979583113)
--(axis cs:17,2.75639969071217)
--(axis cs:16,2.80298590450029)
--(axis cs:15,2.81300492270166)
--(axis cs:14,2.86628845110533)
--(axis cs:13,2.89619715400406)
--(axis cs:12,2.96357246275491)
--(axis cs:11,2.97772705608183)
--(axis cs:10,3.01262832613002)
--(axis cs:9,3.07784065758899)
--(axis cs:8,3.14662513528163)
--(axis cs:7,2.99866669546948)
--(axis cs:6,2.85675127239723)
--(axis cs:5,2.67952074646925)
--(axis cs:4,2.59619387525859)
--(axis cs:3,1.91550612319301)
--(axis cs:2,1.25546406944345)
--(axis cs:1,0.954337164319859)
--(axis cs:0,0.684164572657574)
--cycle;

\path [draw=red, fill=red, opacity=0.3]
(axis cs:0,0.684164572657574)
--(axis cs:0,0.389589783065727)
--(axis cs:1,0.611133092394788)
--(axis cs:2,0.766847364489009)
--(axis cs:3,1.12251192737095)
--(axis cs:4,1.56700731868895)
--(axis cs:5,2.0789618957558)
--(axis cs:6,2.56231856049178)
--(axis cs:7,2.82804153113326)
--(axis cs:8,3.16838993492211)
--(axis cs:9,3.41538131674228)
--(axis cs:10,3.69887097596198)
--(axis cs:11,3.82819514919123)
--(axis cs:12,3.95620363122231)
--(axis cs:13,4.04732020088662)
--(axis cs:14,4.16365582424724)
--(axis cs:15,4.27126121657736)
--(axis cs:16,4.39386518290566)
--(axis cs:17,4.49151489265961)
--(axis cs:18,4.61403736136539)
--(axis cs:19,4.70587684280087)
--(axis cs:20,4.81358139347538)
--(axis cs:21,4.91620373931629)
--(axis cs:22,5.02999599427929)
--(axis cs:23,5.13527221240554)
--(axis cs:24,5.24816103240084)
--(axis cs:25,5.37006832297189)
--(axis cs:26,5.47067324424046)
--(axis cs:27,5.5665012344676)
--(axis cs:28,5.67669998402604)
--(axis cs:29,5.78023186058459)
--(axis cs:30,5.88549736844384)
--(axis cs:31,5.98086100143617)
--(axis cs:32,6.09254880121012)
--(axis cs:33,6.16343106459895)
--(axis cs:34,6.27306674217477)
--(axis cs:35,6.34800122339403)
--(axis cs:36,6.46237350245622)
--(axis cs:37,6.55696935283378)
--(axis cs:38,6.65432334185494)
--(axis cs:39,6.76196754536305)
--(axis cs:40,6.87275016042265)
--(axis cs:41,6.94521667023534)
--(axis cs:42,7.04091234279559)
--(axis cs:43,7.13055919235257)
--(axis cs:44,7.23070233629057)
--(axis cs:45,7.30917631506284)
--(axis cs:46,7.41011376166366)
--(axis cs:47,7.48054904551964)
--(axis cs:48,7.59978499918392)
--(axis cs:49,7.68406976592244)
--(axis cs:50,7.77392232896297)
--(axis cs:51,7.86878674862752)
--(axis cs:52,7.9743248097413)
--(axis cs:53,8.04505955360047)
--(axis cs:54,8.14684816459734)
--(axis cs:55,8.22982804266062)
--(axis cs:56,8.32908460767612)
--(axis cs:57,8.41011680581006)
--(axis cs:58,8.51212451879424)
--(axis cs:59,8.59090087578971)
--(axis cs:60,8.69999531387311)
--(axis cs:61,8.79931468734028)
--(axis cs:62,8.89337603108008)
--(axis cs:63,8.96770079543808)
--(axis cs:64,9.07729869026813)
--(axis cs:65,9.16252080357033)
--(axis cs:66,9.25708064817199)
--(axis cs:67,9.3503631373662)
--(axis cs:68,9.44703598711422)
--(axis cs:69,9.54380515354418)
--(axis cs:70,9.64617959328241)
--(axis cs:71,9.71902763605015)
--(axis cs:72,9.83577871466957)
--(axis cs:73,9.91700845239628)
--(axis cs:74,10.0058004147097)
--(axis cs:75,10.0952697934751)
--(axis cs:76,10.2020770123568)
--(axis cs:77,10.2779827412983)
--(axis cs:78,10.3683859743986)
--(axis cs:79,10.4476346763409)
--(axis cs:80,10.5509789045135)
--(axis cs:81,10.6293307034501)
--(axis cs:82,10.7197613885995)
--(axis cs:83,10.7984646027305)
--(axis cs:84,10.8934122241815)
--(axis cs:85,10.9828983254552)
--(axis cs:86,11.065885132905)
--(axis cs:87,11.1468073353848)
--(axis cs:88,11.2547110952079)
--(axis cs:89,11.3270665504)
--(axis cs:90,11.4184844353945)
--(axis cs:91,11.5034547243957)
--(axis cs:92,11.596826310127)
--(axis cs:93,11.6772795691634)
--(axis cs:94,11.769867883994)
--(axis cs:95,11.8464816672569)
--(axis cs:96,11.9552607046634)
--(axis cs:97,12.0403941418922)
--(axis cs:98,12.1282789632446)
--(axis cs:99,12.2190806914644)
--(axis cs:100,12.3216855735355)
--(axis cs:100,20.4852077123292)
--(axis cs:100,20.4852077123292)
--(axis cs:99,20.2593584280336)
--(axis cs:98,20.0974682944749)
--(axis cs:97,19.9292753535629)
--(axis cs:96,19.7729188181961)
--(axis cs:95,19.5399340434638)
--(axis cs:94,19.4312915228202)
--(axis cs:93,19.2178941150554)
--(axis cs:92,19.0687249845662)
--(axis cs:91,18.8892184703355)
--(axis cs:90,18.7340055694597)
--(axis cs:89,18.5271107617298)
--(axis cs:88,18.4215708238124)
--(axis cs:87,18.1908371720294)
--(axis cs:86,18.0428681033072)
--(axis cs:85,17.8798031689503)
--(axis cs:84,17.7189707391821)
--(axis cs:83,17.5044089971229)
--(axis cs:82,17.3930962977018)
--(axis cs:81,17.1847517100914)
--(axis cs:80,17.0383426081004)
--(axis cs:79,16.8503797332962)
--(axis cs:78,16.7214389230138)
--(axis cs:77,16.5158025891398)
--(axis cs:76,16.4073167608126)
--(axis cs:75,16.1769779404928)
--(axis cs:74,16.0161277861592)
--(axis cs:73,15.8476693253344)
--(axis cs:72,15.6914885695254)
--(axis cs:71,15.4512147926518)
--(axis cs:70,15.3478622520967)
--(axis cs:69,15.1283958563098)
--(axis cs:68,14.9584912252924)
--(axis cs:67,14.7773883257074)
--(axis cs:66,14.6161705858926)
--(axis cs:65,14.40342252655)
--(axis cs:64,14.2873320286387)
--(axis cs:63,14.0757007489721)
--(axis cs:62,13.9368761554469)
--(axis cs:61,13.7637886314759)
--(axis cs:60,13.5916236493281)
--(axis cs:59,13.3642019824886)
--(axis cs:58,13.2554357983719)
--(axis cs:57,13.0366928159749)
--(axis cs:56,12.8862272282403)
--(axis cs:55,12.7034723993606)
--(axis cs:54,12.552188951572)
--(axis cs:53,12.3308688420857)
--(axis cs:52,12.2339841675999)
--(axis cs:51,12.0062066739743)
--(axis cs:50,11.8438769776083)
--(axis cs:49,11.6772211146955)
--(axis cs:48,11.5460540054428)
--(axis cs:47,11.3048356731894)
--(axis cs:46,11.2062037004032)
--(axis cs:45,10.9906185410841)
--(axis cs:44,10.8499044732282)
--(axis cs:43,10.6661853035891)
--(axis cs:42,10.5060115458847)
--(axis cs:41,10.3017592159777)
--(axis cs:40,10.2014622570481)
--(axis cs:39,9.97213475284519)
--(axis cs:38,9.7929975211267)
--(axis cs:37,9.62296061742415)
--(axis cs:36,9.46191448708696)
--(axis cs:35,9.22932576789268)
--(axis cs:34,9.12903240225429)
--(axis cs:33,8.91034425954195)
--(axis cs:32,8.77889264347386)
--(axis cs:31,8.59218128890052)
--(axis cs:30,8.43591508518209)
--(axis cs:29,8.22902207695371)
--(axis cs:28,8.09213910685524)
--(axis cs:27,7.8789510522258)
--(axis cs:26,7.72878887378239)
--(axis cs:25,7.55577043371377)
--(axis cs:24,7.3749306596759)
--(axis cs:23,7.17497072642516)
--(axis cs:22,7.04366710083498)
--(axis cs:21,6.84229559633076)
--(axis cs:20,6.68487826552187)
--(axis cs:19,6.5137232026531)
--(axis cs:18,6.38364106345717)
--(axis cs:17,6.17714672483729)
--(axis cs:16,6.05636824562813)
--(axis cs:15,5.86753273561367)
--(axis cs:14,5.71714477975613)
--(axis cs:13,5.54179786630261)
--(axis cs:12,5.43512563713577)
--(axis cs:11,5.23473868901605)
--(axis cs:10,5.05469656617858)
--(axis cs:9,4.66928847682248)
--(axis cs:8,4.35825125427417)
--(axis cs:7,3.91766091032254)
--(axis cs:6,3.47618881285374)
--(axis cs:5,2.83991561993321)
--(axis cs:4,2.17895996123372)
--(axis cs:3,1.61064796919003)
--(axis cs:2,1.18339488282335)
--(axis cs:1,0.957742087985344)
--(axis cs:0,0.684164572657574)
--cycle;

\addplot [green, mark=triangle, mark size=\markSize, mark options={solid,rotate=180,fill=none}, each nth point=\pointInt]
table {%
0 0.536877155303955
1 0.751457691192627
2 0.990249633789062
3 1.53938400745392
4 2.11267948150635
5 2.1257016658783
6 2.24963665008545
7 2.32354092597961
8 2.4327175617218
9 2.3039984703064
10 2.19091963768005
11 2.11364030838013
12 2.04583644866943
13 1.90767002105713
14 1.83727216720581
15 1.7387467622757
16 1.65820968151093
17 1.5682384967804
18 1.45465064048767
19 1.33671259880066
20 1.21322333812714
21 1.10809087753296
22 1.02126383781433
23 0.92486572265625
24 0.827963590621948
25 0.732901811599731
26 0.629709482192993
27 0.542188763618469
28 0.468575239181519
29 0.382822394371033
30 0.324144840240479
31 0.288663744926453
32 0.199645519256592
33 0.143712759017944
34 0.0607360601425171
35 0.0103020668029785
36 -0.0648444890975952
37 -0.13008975982666
38 -0.210452437400818
39 -0.272133111953735
40 -0.320422410964966
41 -0.380928516387939
42 -0.431917667388916
43 -0.504119396209717
44 -0.546695709228516
45 -0.61021900177002
46 -0.651804089546204
47 -0.692612051963806
48 -0.715009331703186
49 -0.743488430976868
50 -0.774218559265137
51 -0.802194595336914
52 -0.83875560760498
53 -0.871172189712524
54 -0.899997115135193
55 -0.929795503616333
56 -0.949763059616089
57 -0.959390878677368
58 -0.973825693130493
59 -1.00686359405518
60 -1.0181086063385
61 -1.04380071163177
62 -1.05334067344666
63 -1.0597151517868
64 -1.0609267950058
65 -1.0907233953476
66 -1.09543406963348
67 -1.12777137756348
68 -1.14358568191528
69 -1.1535382270813
70 -1.16458821296692
71 -1.1927205324173
72 -1.20915448665619
73 -1.21205627918243
74 -1.22248005867004
75 -1.23998606204987
76 -1.26284515857697
77 -1.27180790901184
78 -1.28516840934753
79 -1.30666255950928
80 -1.32029402256012
81 -1.3233984708786
82 -1.34301173686981
83 -1.35258328914642
84 -1.36476421356201
85 -1.36883962154388
86 -1.38534224033356
87 -1.39636147022247
88 -1.40587484836578
89 -1.40787792205811
90 -1.42613935470581
91 -1.43171286582947
92 -1.43591594696045
93 -1.43970334529877
94 -1.45170652866364
95 -1.4654848575592
96 -1.47750544548035
97 -1.47664546966553
98 -1.48718428611755
99 -1.49992513656616
100 -1.51749193668365
};
\addlegendentry{DMABO}
\addplot [red, mark=o, mark size=\markSize, mark options={solid,fill=none}, each nth point=\pointInt]
table {%
0 0.536877155303955
1 0.784437656402588
2 0.975121140480042
3 1.36657989025116
4 1.87298369407654
5 2.45943880081177
6 3.01925373077393
7 3.37285113334656
8 3.76332068443298
9 4.04233503341675
10 4.37678384780884
11 4.53146696090698
12 4.69566440582275
13 4.79455900192261
14 4.94040012359619
15 5.06939697265625
16 5.22511672973633
17 5.33433103561401
18 5.49883937835693
19 5.60979986190796
20 5.7492299079895
21 5.87924957275391
22 6.03683137893677
23 6.15512132644653
24 6.31154584884644
25 6.46291923522949
26 6.59973096847534
27 6.72272634506226
28 6.88441944122314
29 7.00462675094604
30 7.16070604324341
31 7.28652095794678
32 7.43572092056274
33 7.53688764572144
34 7.7010498046875
35 7.78866338729858
36 7.96214389801025
37 8.08996486663818
38 8.22366046905518
39 8.36705112457275
40 8.53710651397705
41 8.62348747253418
42 8.77346229553223
43 8.89837265014648
44 9.04030323028564
45 9.14989757537842
46 9.30815887451172
47 9.39269256591797
48 9.57291984558105
49 9.68064498901367
50 9.80889987945557
51 9.93749713897705
52 10.104154586792
53 10.1879644393921
54 10.3495187759399
55 10.4666500091553
56 10.6076555252075
57 10.7234048843384
58 10.8837804794312
59 10.9775514602661
60 11.145809173584
61 11.281551361084
62 11.4151258468628
63 11.5217008590698
64 11.682315826416
65 11.7829713821411
66 11.9366254806519
67 12.0638761520386
68 12.2027635574341
69 12.3361005783081
70 12.4970207214355
71 12.5851211547852
72 12.7636337280273
73 12.8823385238647
74 13.0109643936157
75 13.1361236572266
76 13.3046970367432
77 13.3968925476074
78 13.5449123382568
79 13.6490068435669
80 13.7946605682373
81 13.9070415496826
82 14.0564289093018
83 14.1514368057251
84 14.306191444397
85 14.4313507080078
86 14.5543766021729
87 14.6688222885132
88 14.8381404876709
89 14.9270887374878
90 15.0762453079224
91 15.1963367462158
92 15.3327760696411
93 15.4475870132446
94 15.6005792617798
95 15.6932077407837
96 15.8640899658203
97 15.9848346710205
98 16.1128730773926
99 16.2392196655273
100 16.4034461975098
};
\addlegendentry{DCEI}
\end{axis}

\end{tikzpicture}

